On the Local Controllability of a Class of Quadratic Systems

The local controllability of a rich class of affine nonlinear control systems with nonhomogeneous quadratic drift and constant control vector fields is analyzed. The interest in this particular class of systems stems from the ubiquity in science and engineering of some of its notable representatives, namely the Sprott system, the Lorenz system and the rigid body among others. A necessary and sufficient condition for strong accessibility reminiscent of the Kalman rank condition is derived, and it generalizes Crouch's condition for the rigid body. This condition is in general not sufficient to infer small-time local controllability. However, under some additional mild assumptions local controllability is established. In particular for the Sprott and Lorenz systems, sharp conditions for small-time local controllability are obtained in the single-input case.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}
